Higgs Boson Production at Hadron Colliders at N3LO in QCD

We present the Higgs boson production cross section at Hadron colliders in the gluon fusion production mode through N3LO in perturbative QCD. Specifically, we work in an effective theory where the top quark is assumed to be infinitely heavy and all other quarks are considered to be massless. Our result is the first exact formula for a partonic hadron collider cross section at N3LO in perturbative QCD. Furthermore, this result represents the first analytic computation of a hadron collider cross section involving elliptic integrals. We derive numerical predictions for the Higgs boson cross section at the LHC. Previously this result was approximated by an expansion of the cross section around the production threshold of the Higgs boson and we compare our findings. Finally, we study the impact of our new result on the state of the art prediction for the Higgs boson cross section at the LHC.

==> Chapters/APP_SV.tex <==
\section{The Soft-Virtual Cross Section at N$^3$LO}


\bea
\eta_{ij}^{(n),\text{ SV}}(z)&=&
8 D_5 n_c^3\nonumber\\
&+&\left(20 L n_c^3-\frac{110 n_c^3}{9}+\frac{20 n_f n_c^2}{9}\right) D_4\nonumber\\
&+&\left(16 L^2 n_c^3+\frac{1}{27} \left(925-252 \pi ^2\right) n_c^3-\frac{164 n_f n_c^2}{27}+\frac{4 n_f^2 n_c}{27}\right.\nonumber\\
&+&\left.L \left(\frac{40 n_c^2 n_f}{9}-\frac{220 n_c^3}{9}\right)\right) D_3\nonumber\\
&+&D_2 \left(4 L^3 n_c^3+\frac{1}{54} \left(-2102+561 \pi ^2+9774 \zeta (3)\right) n_c^3-\frac{10 n_f^2 n_c}{27}\right.\nonumber\\
&+&\left. L^2 \left(3 n_c^2 n_f-\frac{33 n_c^3}{2}\right)+L \left(\frac{1}{18} \left(925-252 \pi ^2\right) n_c^3-\frac{82 n_f n_c^2}{9}+\frac{2 n_f^2 n_c}{9}\right)\right.\nonumber\\
&+&\left.n_f \left(\frac{1}{108} n_c^2 \left(941-204 \pi ^2\right)-\frac{1}{4}\right)\right)\nonumber\\
&+&D_1 \left(\left(\frac{2 n_c^2 n_f}{3}-\frac{11 n_c^3}{3}\right) L^3+\left(\frac{1}{4} \left(73-24 \pi ^2\right) n_c^3-\frac{31 n_f n_c^2}{9}+\frac{n_f^2 n_c}{9}\right) L^2\right.\nonumber\\
&+&\left.\left(\frac{1}{18} \left(-674+143 \pi ^2+3240 \zeta (3)\right) n_c^3-\frac{10 n_f^2 n_c}{27}+n_f \left(\frac{1}{108} n_c^2 \left(1099-156 \pi ^2\right)-\frac{3}{4}\right)\right) L\right.\nonumber\\
&+&\left.n_f \left(\frac{n_c^2 \left(-21947+2256 \pi ^2+23760 \zeta (3)\right)}{1296}-\frac{3}{16} (-21+16 \zeta (3))\right)\right.\nonumber\\
&+&\left.\frac{n_c^3 \left(152845-27360 \pi ^2-2772 \pi ^4-380160 \zeta (3)\right)}{3240}+\frac{1}{81} n_c n_f^2 \left(25-6 \pi ^2\right)\right)\nonumber\\
&+&D_0 \left(\left(-\frac{1}{216} (-11+12 \pi ) (11+12 \pi ) n_c^3-\frac{11 n_f n_c^2}{54}+\frac{n_f^2 n_c}{54}\right) L^3\right.\nonumber\\
&+&\left.\left(\frac{1}{216} \left(-1538+231 \pi ^2+7560 \zeta (3)\right) n_c^3-\frac{5 n_f^2 n_c}{54}+n_f \left(\frac{1}{432} n_c^2 \left(1145-84 \pi ^2\right)-\frac{5}{16}\right)\right) L^2+\left(\frac{\left(152845-27360 \pi ^2-2772 \pi ^4-380160 \zeta (3)\right) n_c^3}{6480}+\frac{1}{162} n_f^2 \left(25-6 \pi ^2\right) n_c+n_f \left(\frac{n_c^2 \left(-21947+2256 \pi ^2+23760 \zeta (3)\right)}{2592}-\frac{3}{32} (-21+16 \zeta (3))\right)\right) L+n_f \left(\frac{\left(171449-54096 \pi ^2-864 \pi ^4-640224 \zeta (3)\right) n_c^2}{46656}+\frac{-8555+360 \pi ^2+24 \pi ^4+4560 \zeta (3)}{8640}\right)+\frac{n_c^3 \left(-1485145+513780 \pi ^2+13662 \pi ^4+9656280 \zeta (3)-2349000 \pi ^2 \zeta (3)+21695040 \zeta (5)\right)}{116640}+\frac{1}{729} n_c n_f^2 \left(-58+45 \pi ^2+135 \zeta (3)\right)\right)\nonumber\\
&+&\delta(1-z)\left(\left(\frac{1}{36} n_c^3 \left(11 \pi ^2+96 \zeta (3)\right)-\frac{1}{18} n_c^2 n_f \pi ^2\right) L^3+\left(\frac{\left(2970-2075 \pi ^2-216 \pi ^4-26730 \zeta (3)\right) n_c^3}{2160}+n_f^2 \left(\frac{1}{432} n_c \left(45+4 \pi ^2\right)-\frac{1}{48 n_c}\right)+n_f \left(\frac{1}{96} \left(-79+8 \pi ^2+216 \zeta (3)\right) n_c^2+\frac{11}{96}\right)\right) L^2+\left(\frac{\left(-74556-3176 \pi ^2-165 \pi ^4+226872 \zeta (3)-52272 \pi ^2 \zeta (3)+484704 \zeta (5)\right) n_c^3}{5184}+n_f \left(\frac{\left(14919+844 \pi ^2+10 \pi ^4-12816 \zeta (3)\right) n_c^2}{1728}+\frac{1}{96} \left(-151-6 \pi ^2+88 \zeta (3)\right)-\frac{1}{64 n_c^2}\right)+n_f^2 \left(\frac{\left(-2367-80 \pi ^2+288 \zeta (3)\right) n_c}{2592}+\frac{13-8 \zeta (3)}{48 n_c}\right)\right) L+n_f^2 \left(\frac{\left(90195-3695 \pi ^2-234 \pi ^4-7200 \zeta (3)\right) n_c}{38880}+\frac{-22405+690 \pi ^2+4 \pi ^4+15120 \zeta (3)}{25920 n_c}\right)+n_f \left(\frac{\left(-3860595-47960 \pi ^2+10648 \pi ^4+1511640 \zeta (3)-231120 \pi ^2 \zeta (3)+1877040 \zeta (5)\right) n_c^2}{155520}+\frac{292595+8520 \pi ^2-44 \pi ^4-248400 \zeta (3)-12960 \pi ^2 \zeta (3)+64800 \zeta (5)}{51840}+\frac{38+111 \zeta (3)-180 \zeta (5)}{144 n_c^2}\right)+\frac{n_c^3 \left(22588755+1130570 \pi ^2-106799 \pi ^4-24036 \pi ^6-27862380 \zeta (3)+3700620 \pi ^2 \zeta (3)+37467360 \zeta (3)^2-28648620 \zeta (5)\right)}{544320}\right)
\eea

